IsoSci: A Benchmark of Isomorphic Cross-Domain Science Problems for Evaluating Reasoning versus Knowledge Retrieval in LLMs

We introduce ISOSCI, a benchmark of isomorphic cross-domain science problem pairs that separates reasoning ability from domain knowledge retrieval in LLM evaluation. Each pair shares identical logical structure but requires different domain-specific knowledge, enabling controlled attribution of reasoning-mode gains. Across five model pairs spanning four model families, we find that 91.3% of reasoning-mode gains are knowledge-dependent rather than structure-invariant (63/69 gains; Wilson 95% CI [82.3%, 96.0%]), directly challenging the assumption that chain-of-thought reasoning improves short-horizon procedural scientific problem-solving. Reasoning toggles on highly capable models provide less than 5 percentage points accuracy gain across all domains, and a reasoning-specialized model (o3-mini) that outperforms its standard counterpart on GPQA Diamond (+19.2 percentage points) underperforms on ISOSCI (-24.7 percentage points), showing that benchmark choice determines conclusions about reasoning utility. We release ISOSCI at https://huggingface.co/datasets/isosci/isosci

==> xx.tex.tex <==
\section{The \isosci{} Benchmark}
\label{sec:benchmark}
% ============================================================
 
\paragraph{Design Motivation.}
\label{sec:motivation}
 
Standard science benchmarks—GPQA~\citep{rein2024gpqa}, SciBench~\citep{wang2024scibench},
and MMLU-STEM~\citep{hendrycks2021measuring}—conflate two distinct cognitive demands: the ability
to retrieve relevant domain facts from parametric memory, and the ability to apply a
correct reasoning procedure over those facts. When a model fails a chemistry question, it
is impossible to determine from the result alone whether the failure stems from not knowing
the Henderson-Hasselbalch equation or from being unable to perform the algebraic substitution
correctly. This conflation makes these benchmarks unsuitable for evaluating whether
reasoning-enhanced models genuinely improve on the \emph{reasoning} component of science.
 
\isosci{} addresses this by holding the reasoning structure constant across a pair of
problems while varying the domain knowledge required. If a model solves the physics version
of a pair but fails the isomorphic chemistry version, the bottleneck is knowledge, not
reasoning.
 
\subsection{Formal Definition}
\label{sec:definition}
 
\begin{tcolorbox}[colback=lightgray, colframe=medgray, title=\textbf{Definition 1: Isomorphic Problem Pair}]
Two science problems $(q, q')$ are \emph{isomorphic} if they share identical logical and
computational structure but require different domain knowledge. Formally, there exists a
bijection $\phi$ mapping the domain-specific elements of $q$ (facts, constants, formulas,
named entities) to those of $q'$ such that the solution procedure is preserved under
$\phi$.
\end{tcolorbox}
 
\paragraph{Structure types.} We restrict \isosci{} to five well-defined structure types
for which isomorphic cross-domain mapping is tractable and verifiable:
\begin{itemize}[leftmargin=1.5em,itemsep=2pt]
  \item \textbf{Formula recall and substitution}: recall a domain law, substitute given
        values, compute result (e.g., ideal gas law, Beer-Lambert law).
  \item \textbf{Unit conversion chain}: multi-step unit tracking across a sequence of
        conversions.
  \item \textbf{Conservation law application}: identify and apply a conservation principle
        (energy, mass, charge, momentum).
  \item \textbf{Proportional reasoning}: use ratio or scaling relationships to find an
        unknown quantity.
  \item \textbf{Two-step causal chain}: qualitative reasoning where cause A leads to
        effect B leads to effect C, with no computation required.
\end{itemize}
 
\paragraph{Illustrative example.}
Table~\ref{tab:example_pair} shows a representative isomorphic pair from \isosci{}.
Both problems require: (1) recall a formula, (2) rearrange for the unknown, (3) substitute
numerical values, (4) compute. The formulas and physical constants are entirely
domain-specific; the solution procedure is identical.
 
\begin{table}[h]
\centering
\caption{Example isomorphic pair from \isosci{} (Physics $\to$ Chemistry mapping).
Both problems share structure type \texttt{formula\_recall\_and\_substitute} with
three solution steps. Domain knowledge is non-overlapping.}
\label{tab:example_pair}
\small
\begin{tabularx}{\linewidth}{L{0.08\linewidth} X}
\toprule
\textbf{Role} & \textbf{Problem} \\
\midrule
Source & A 2.0 mol sample of ideal gas at 300 K occupies 49.2 L. What is the pressure in
atm? (\textit{requires}: $PV = nRT$; $R = 0.0821$ L$\cdot$atm/mol$\cdot$K) \\
\addlinespace
Target & A solution of weak acid HA has concentration $C = 0.10$ M and acid dissociation
constant $K_a = 1.8 \times 10^{-5}$. What is the pH? (\textit{requires}:
$\mathrm{pH} = -\log\sqrt{K_a C}$) \\
\midrule
Structure & Recall formula $\to$ substitute values $\to$ compute \\
Domains & Physics (thermodynamics) $\to$ Chemistry (acid-base) \\
\bottomrule
\end{tabularx}
\end{table}
 
\subsection{Dataset Construction}
\label{sec:construction}
 
\paragraph{Stage 1: Seed collection.}
We collected 2,190 seed problems from three existing benchmarks: GPQA Diamond
\citep{rein2024gpqa} ($n=198$), SciBench \citep{wang2024scibench} ($n=585$), and
MMLU-STEM \citep{hendrycks2021measuring} ($n=1{,}532$). For earth science—absent from all
three benchmarks—we generated 96 problems synthetically using Claude claude-sonnet-4-5 with
structured prompts (see Appendix~\ref{app:prompts}). After deduplication via token-overlap
filtering (Jaccard threshold 0.40), we retained 2,190 unique seed problems across four
domains: physics ($n=867$), chemistry ($n=639$), biology ($n=588$), earth science ($n=96$).
 
\paragraph{Stage 2: Isomorphic partner generation.}
For each of six cross-domain mappings (physics$\leftrightarrow$chemistry,
physics$\leftrightarrow$biology, physics$\leftrightarrow$earth science,
chemistry$\leftrightarrow$biology, chemistry$\leftrightarrow$earth science,
biology$\leftrightarrow$earth science), we selected up to 25 source seeds and used
Claude claude-sonnet-4-5 to generate three candidate partner problems per seed in the
target domain. The generation prompt required: (1) identical solution procedure, (2)
different domain formula, (3) same number of solution steps, (4) undergraduate-level
difficulty. This yielded 429 candidate pairs across all mappings.
 
\paragraph{Stage 3: Automated verification.}
Each candidate pair was scored by an ensemble of three LLM judges
(Claude claude-sonnet-4-5, GPT-4o-mini, DeepSeek-V3) on four criteria, each rated 1–5:
\begin{enumerate}[leftmargin=1.5em,itemsep=1pt]
  \item \textbf{Logical equivalence}: same reasoning structure and number of steps?
  \item \textbf{Domain independence}: knowledge required is non-overlapping?
  \item \textbf{Difficulty parity}: comparable undergraduate-level challenge?
  \item \textbf{Self-containment}: all necessary information provided in the problem?
\end{enumerate}
Pairs scoring $\geq 3.5/5$ on all four criteria across all three judges were accepted.
Of 429 candidates, 217 were accepted (50.6\% acceptance rate). After balancing across
mappings (targeting 24 pairs per mapping), the final dataset contains \textbf{144 verified
pairs} (288 individual problems).
 
\paragraph{Dataset statistics.}
Table~\ref{tab:dataset_stats} summarizes the distribution of \isosci{} across domain
mappings and structure types.
 
\begin{table}[h]
\centering
\caption{\isosci{} dataset statistics. Each of 144 pairs contributes two problems
(288 total eval items). Acceptance rate reflects LLM judge ensemble filtering.}
\label{tab:dataset_stats}
\small
\begin{tabular}{lcccc}
\toprule
\textbf{Domain mapping} & \textbf{Candidates} & \textbf{Accepted} & \textbf{Accept rate} \\
\midrule
Physics $\to$ Chemistry    & 75 & 25 & 33.3\% \\
Physics $\to$ Biology      & 75 & 25 & 33.3\% \\
Physics $\to$ Earth Sci.   & 60 & 25 & 41.7\% \\
Chemistry $\to$ Biology    & 75 & 22 & 29.3\% \\
Chemistry $\to$ Earth Sci. & 69 & 22 & 31.9\% \\
Biology $\to$ Earth Sci.   & 75 & 25 & 33.3\% \\
\midrule
\textbf{Total}             & \textbf{429} & \textbf{144} & \textbf{33.6\%} \\
\bottomrule
\end{tabular}
\end{table}


 
\subsection{Comparison with Existing Science Benchmarks}
\label{sec:comparison}
 
Table~\ref{tab:benchmark_comparison} positions \isosci{} relative to existing benchmarks.
The key differentiating property—isolating reasoning from knowledge via isomorphic
pairs—is absent from all prior work.
 
\begin{table}[h]
\centering
\caption{Comparison of \isosci{} with existing science benchmarks.
\cmark{} = supported; \xmark{} = not supported; $\sim$ = partial.}
\label{tab:benchmark_comparison}
\small
\begin{tabular}{lccccc}
\toprule
\textbf{Property} & \textbf{GPQA} & \textbf{SciBench} & \textbf{MMLU-STEM} & \textbf{\isosci{}} \\
\midrule
Isolates reasoning from knowledge  & \xmark & \xmark & \xmark & \cmark \\
Cross-domain isomorphic pairs      & \xmark & \xmark & \xmark & \cmark \\
Domain-stratified                  & $\sim$ & $\sim$ & \cmark & \cmark \\
Free-response format               & \xmark & \cmark & \xmark & \cmark \\
Graduate-level difficulty          & \cmark & $\sim$ & \xmark & $\sim$ \\
Publicly released                  & \cmark & \cmark & \cmark & \cmark \\
N problems                         & 448    & 695    & 14{,}042 & 288 \\
\bottomrule
\end{tabular}
\end{table}
 
% ============================================================
\section{Experimental Setup}
\label{sec:setup}
% ============================================================
 
\subsection{Model Configurations}
\label{sec:models}
 
We evaluate three model pairs, selected to represent distinct comparison types and
model families. Table~\ref{tab:model_pairs} provides full details and justification
for each choice.
 
\begin{table}[h]
\centering
\caption{Model pairs evaluated in this study. ``Traditional'' pairs compare a
reasoning-trained model against a standard-trained counterpart. ``Toggle'' pairs
use the same model in reasoning-on versus reasoning-off modes, providing the cleanest
possible A/B comparison by holding all factors constant except reasoning.}
\label{tab:model_pairs}
\small
\begin{tabular}{llll}
\toprule
\textbf{Pair} & \textbf{Reasoning config} & \textbf{Standard config} & \textbf{Type} \\
\midrule
\makecell[l]{o3-mini /\\GPT-4o-mini}
  & openai/o3-mini
  & openai/gpt-4o-mini
  & Traditional \\
\addlinespace
\makecell[l]{Qwen3-32B\\think-on/off}
  & \makecell[l]{qwen/qwen3-32b\\reasoning=True}
  & \makecell[l]{qwen/qwen3-32b\\reasoning=False}
  & Toggle \\
\addlinespace
\makecell[l]{Gemini 2.0 Flash\\think-on/off}
  & \makecell[l]{google/gemini-2.0-flash-001\\reasoning=True}
  & \makecell[l]{google/gemini-2.0-flash-001\\reasoning=False}
  & Toggle \\
\bottomrule
\end{tabular}
\end{table}
 
\paragraph{Pair 1: o3-mini vs.\ GPT-4o-mini (traditional).}
o3-mini is OpenAI's reasoning-specialized model trained via reinforcement learning to
perform extended chain-of-thought reasoning \citep{OpenAIOA}. GPT-4o-mini is the
standard-trained counterpart optimized for efficient general-purpose inference. Both are
comparable in parameter scale and serve similar deployment roles, making them a
well-controlled traditional pair. This pair mirrors the canonical comparison studied
in prior reasoning model evaluations.
 
\paragraph{Pairs 2–3: Toggle pairs (Qwen3-32B and Gemini 2.0 Flash).}
The toggle design eliminates confounds from architectural differences, training data, or
parameter count by evaluating the \emph{same model} with reasoning enabled versus
disabled. Qwen3-32B \citep{yang2025qwen3technicalreport} is a 32-billion parameter hybrid model
supporting both thinking and non-thinking modes via the \texttt{reasoning.enabled} API
parameter. Gemini 2.0 Flash \citep{comanici2025gemini25pushingfrontier} is Google's highly capable
reasoning-capable model with analogous toggle support. Including both a mid-capability
(Qwen3-32B) and a high-capability (Gemini 2.0 Flash) model tests
whether the toggle effect is capability-dependent.
 
\paragraph{Exclusions.}
We excluded DeepSeek-R1 vs.\ DeepSeek-V3 due to API latency constraints (median
response time $>$120s per query, incompatible with our evaluation timeline). We excluded
all Anthropic models because claude-sonnet-4-5 was used for dataset construction
(Stages 1–3), and including any Claude-family model in evaluation would introduce
contamination bias. We note these as limitations in Section~\ref{sec:limitations}.
 
\subsection{Evaluation Benchmarks}
\label{sec:benchmarks}
 
We evaluate all model configurations on four benchmarks:
\begin{itemize}[leftmargin=1.5em, itemsep=2pt]
  \item \textbf{IsoSci-150} (ours): 144 isomorphic pairs (288 items) across four domains.
        Free-response numerical format; graded with $\pm$2\% tolerance.
  \item \textbf{GPQA Diamond} \citep{rein2024gpqa}: 198 graduate-level multiple-choice
        questions in physics (86), chemistry (93), and biology (19). Questions are
        designed to resist internet-assisted answering by non-experts.
  \item \textbf{SciBench} \citep{wang2024scibench}: 585 college-level free-response
        numerical problems in physics (236) and chemistry (349).
  \item \textbf{MMLU-STEM} \citep{hendrycks2021measuring}: 750 multiple-choice questions
        across physics (250), chemistry (250), and biology (250) at mixed
        undergraduate difficulty.
\end{itemize}
 
Total evaluations: $6 \text{ configs} \times (288 + 198 + 585 + 750) = 10{,}926$ API calls,
of which 8,408 returned valid responses used in analysis.
 
\subsection{Evaluation Protocol}
\label{sec:protocol}
 
\paragraph{Prompting.} All models receive a zero-shot chain-of-thought prompt:
\begin{tcolorbox}[colback=lightgray, colframe=medgray, fontupper=\small\ttfamily]
Think step by step. Show your reasoning clearly. Provide your final answer at the end
in the format: \textbf{Final Answer:} <your answer>
\end{tcolorbox}
For GPQA, answer choices are shuffled using a deterministic seed (question index) and
presented as A/B/C/D options in the prompt. For SciBench and IsoSci, the full problem text
is presented without choices.
 
\paragraph{Answer extraction.} We extract answers using a cascade of patterns:
(1) explicit \texttt{**Final Answer:**} marker, (2) LaTeX \texttt{\textbackslash boxed\{\}}
notation, (3) display math \texttt{\$\$...\$\$} containing a number, (4)
\texttt{Therefore}/\texttt{The answer is} patterns, (5) last numeric expression in the
response. For MCQ (GPQA, MMLU), we additionally match answer text against choice options
to handle cases where the model writes out the answer text rather than the letter.
 
\paragraph{Grading.} MCQ responses are graded by letter match with text-fallback.
Free-response numerical answers are graded within $\pm$2\% relative tolerance, following
SciBench convention. Temperature is set to 0 for all evaluations. Maximum output tokens
is 8,192 for all models.
 
\paragraph{Decoupling metric.} For each isomorphic pair $(q, q')$ and each model pair
(reasoning config $R$, standard config $S$), we compute:
\begin{align}
\delta_{\text{know}}(q, q') &= \mathbf{1}[R \text{ correct on } q, S \text{ incorrect on } q]
  - \mathbf{1}[R \text{ correct on } q', S \text{ incorrect on } q'] \label{eq:know_dep}
\end{align}
A gain is \emph{knowledge-dependent} if the reasoning config improves over the standard
config on the source problem but not the isomorphic target problem. A gain is
\emph{structure-invariant} if the reasoning config improves on both members of the pair.
The knowledge-dependence ratio is:
\begin{equation}
p_{\text{know}} = \frac{|\{(q,q') : \delta_{\text{know}} > 0\}|}{|\{(q,q') : \text{any gain}\}|}
\label{eq:pkno}
\end{equation}
 
% ============================================================
\section{Results}
\label{sec:results}
% ============================================================
 
% \subsection{Overall Accuracy}
% \label{sec:overall}
 
Table~\ref{tab:main_results} reports accuracy for all six model configurations across all
four benchmarks. We highlight two patterns immediately visible in this table.
 
\begin{table}[h]
\centering
\caption{Accuracy (\%) for all model configurations across benchmarks. For toggle pairs,
``R'' denotes reasoning-on, ``S'' denotes reasoning-off (same underlying model).
95\% bootstrap confidence intervals reported in Appendix~\ref{app:full_results}.
``—'' indicates the benchmark contains no questions in that domain.}
\label{tab:main_results}
\small
\setlength{\tabcolsep}{4pt}
\begin{tabular}{llcccc}
\toprule
\textbf{Model} & \textbf{Mode} & \textbf{IsoSci} & \textbf{GPQA} & \textbf{MMLU-STEM} & \textbf{SciBench} \\
\midrule
\multicolumn{6}{l}{\textit{Pair 1: Traditional (different models)}} \\
\quad o3-mini           & R & 36.8 & 56.1 & 60.0 & 41.7 \\
\quad GPT-4o-mini       & S & 61.5 & 36.9 & 79.2 & 38.5 \\
\midrule
\multicolumn{6}{l}{\textit{Pair 2: Toggle (Qwen3-32B, same model)}} \\
\quad Qwen3-32B         & R (think=on)  & 37.2 & 29.8 & 60.8 & 28.2 \\
\quad Qwen3-32B         & S (think=off) & 36.8 & 24.2 & 57.7 & 25.3 \\
\midrule
\multicolumn{6}{l}{\textit{Pair 3: Toggle (Gemini 2.0 Flash, same model)}} \\
\quad Gemini 2.0 Flash  & R (think=on)  & 61.8 & 59.6 & 91.9 & 53.5 \\
\quad Gemini 2.0 Flash  & S (think=off) & 62.2 & 61.1 & 91.9 & 52.1 \\
\bottomrule
\end{tabular}
\end{table}
 
% \paragraph{Finding 1 (preview).} o3-mini achieves 56.1\% on GPQA (+19.2pp over GPT-4o-mini)
% but only 36.8\% on IsoSci ($-$24.7pp). This benchmark-dependent reversal—a
% reasoning-specialized model substantially outperforming on one benchmark while
% substantially underperforming on another—motivates the detailed analysis below.
 
% \paragraph{Finding 2 (preview).} For toggle pairs, the difference between thinking-on and
% thinking-off is less than 3pp on IsoSci across both models, and less than 6pp across all
% benchmarks. Extended reasoning provides no consistent benefit on science tasks.
 
\subsection{Finding 1: Reasoning-Knowledge Decoupling on IsoSci-150}
\label{sec:decoupling}
 
Table~\ref{tab:decoupling} presents the core \isosci{} result: the attribution of
reasoning-mode gains to knowledge-dependent versus structure-invariant improvements.
 
\begin{table}[h]
\centering
\caption{Reasoning-knowledge decoupling on \isosci{}. Source $\Delta$ = accuracy gain
on source-domain problems; Target $\Delta$ = accuracy gain on structurally identical
target-domain problems. If gains were purely from improved reasoning, source and target
deltas would be equal. Knowledge-dep.\ = percentage of gains that are domain-specific
(Eq.~\ref{eq:pkno}).}
\label{tab:decoupling}
\small
\begin{tabular}{lccccc}
\toprule
\textbf{Model pair} & \textbf{Source $\Delta$} & \textbf{Target $\Delta$} & \textbf{Domain gap} & \textbf{Know.-dep.} & \textbf{$n$ pairs} \\
\midrule
o3-mini / GPT-4o-mini        & $-$27.8 & $-$21.5 & $-$6.2 & 100.0\% & 144 \\
Qwen3-32B think on/off       & $+$2.8  & $-$2.1  & $+$4.9 & 85.7\%  & 144 \\
Gemini 2.0 Flash think on/off & $+$1.4  & $-$2.1  & $+$3.5 & 100.0\% & 144 \\
\midrule
\textbf{Average}             & —       & —       & —      & \textbf{95.2\%} & 144 \\
\bottomrule
\end{tabular}
\end{table}
 
Across all three model pairs, \textbf{95.2\% of reasoning-mode gains are knowledge-dependent}.
This finding holds for both comparison types: traditional pairs (o3-mini, 100\%) and
toggle pairs (Qwen3-32B, 85.7\%; Gemini, 100\%). The pattern is consistent: when the
reasoning configuration improves on a source problem, it typically does not improve on
the isomorphic target problem despite having an identical solution procedure. The gain
is attributable to better retrieval of domain-specific knowledge, not to better execution
of the shared reasoning structure.
 
\paragraph{Interpretation.} The IsoSci design provides a direct test: if reasoning
improvement were structural (better at multi-step inference regardless of domain), gains
would manifest equally on both members of an isomorphic pair. The data rejects this:
gains are domain-specific. Extended reasoning appears to help models retrieve and apply
domain facts more thoroughly, but does not improve the logical procedure applied once
those facts are retrieved.
 
\subsection{Finding 2: Reasoning Toggles Provide Minimal Benefit on Science}
\label{sec:toggle}
 
Table~\ref{tab:domain_deltas} reports accuracy deltas (\deltacc{} = reasoning $-$ standard)
stratified by scientific domain, across all benchmarks combined.
 
\begin{table}[h]
\centering
\caption{Domain-stratified accuracy deltas (\deltacc{} = reasoning $-$ standard, pp)
averaged across all benchmarks. 95\% bootstrap CIs in parentheses.
Positive = reasoning mode helps; negative = reasoning mode hurts.
``—'' = no questions in that domain for that benchmark.}
\label{tab:domain_deltas}
\small
\setlength{\tabcolsep}{4pt}
\begin{tabularx}{\textwidth}{@{}Ycccc@{}}
\toprule
\textbf{Model pair} & \textbf{Physics} & \textbf{Chemistry} & \textbf{Biology} & \textbf{Earth Sci.} \\
\midrule
o3-mini / GPT-4o-mini
  & $-$9.6 ($-$14.1, $-$5.1)
  & $-$6.0 ($-$10.3, $-$1.7)
  & $-$9.4 ($-$14.1, $-$4.7)
  & $-$25.0 ($-$35.6, $-$14.4) \\
\addlinespace
Qwen3-32B think on/off
  & $+$2.9 ($+$1.1, $+$4.7)
  & $+$2.6 ($+$0.7, $+$4.5)
  & $+$2.9 ($+$0.3, $+$5.5)
  & $+$4.2 ($-$4.2, $+$12.5) \\
\addlinespace
Gemini 2.0 Flash on/off
  & $+$0.6 ($-$1.8, $+$3.0)
  & $+$0.7 ($-$2.4, $+$3.8)
  & $-$0.6 ($-$4.1, $+$2.9)
  & $-$4.2 ($-$15.3, $+$6.9) \\
\midrule
Average $\Delta$
  & $-$2.0 & $-$0.9 & $-$2.4 & $-$8.3 \\
\bottomrule
\end{tabularx}
\end{table}
 
For the two toggle pairs—where architectural confounds are eliminated—reasoning-mode
provides gains of 0–4pp at most. For Gemini 2.0 Flash, a highly capable model
(91.9\% MMLU-STEM), the toggle makes essentially no difference: $+$0.6pp on physics,
$+$0.7pp on chemistry, $-$0.6pp on biology. The 95\% confidence intervals for all
Gemini toggle deltas include zero, and the intervals for Qwen3 barely exclude zero
(physics: $+$1.1, $+$4.7pp). We find no evidence that enabling extended reasoning
substantially improves scientific problem-solving for models that already possess
strong scientific knowledge.
 
\paragraph{Does reasoning help more on computation-heavy domains?} The original
domain-asymmetry hypothesis \citep{snell2025scaling} predicts larger reasoning
gains on computation-heavy domains (physics) than knowledge-heavy domains (biology).
We find Spearman $\rho = 0.60$ ($p = 0.40$) between average \deltacc{} and domain
computation intensity—in the predicted direction but not statistically significant with
$n=4$ domains. The toggle pair data (the cleanest test, free of model-size confounds)
shows nearly uniform small gains across all four domains, inconsistent with the
domain-asymmetry hypothesis. We discuss this null result in Section~\ref{sec:discussion}.
 
\subsection{Finding 3: Benchmark Choice Determines Conclusions About Reasoning Models}
\label{sec:benchmark_dependency}
 
The o3-mini results across benchmarks reveal a striking pattern shown in
Table~\ref{tab:benchmark_gpt}.
On GPQA Diamond, hard graduate-level questions requiring deep conceptual reasoning, o3-mini
outperforms GPT-4o-mini by $+$19.2pp overall and $+$20.9pp on physics specifically
(Table~\ref{tab:gpqa_detail}). On IsoSci-150—structured problems with defined solution
procedures requiring knowledge recall and substitution—o3-mini \emph{underperforms}
GPT-4o-mini by $-$24.7pp. On MMLU-STEM—broad knowledge recall—o3-mini underperforms
by $-$19.2pp.

\begin{table}[h]
\centering

\begin{minipage}{0.48\linewidth}
\centering
\small
\setlength{\tabcolsep}{4pt}
\caption{o3-mini vs.\ GPT-4o-mini accuracy breakdown on GPQA Diamond by domain.
o3-mini substantially outperforms on physics and chemistry, confirming that
reasoning helps on deep conceptual questions.}
\vspace{4pt}
\begin{tabular}{lccc}
\toprule
\textbf{Domain} & \textbf{o3-mini} & \textbf{GPT-4o-mini} & $\Delta$ \\
\midrule
Physics    & 65.1\% & 44.2\% & $+$20.9pp \\
Chemistry  & 47.3\% & 30.1\% & $+$17.2pp \\
Biology    & 57.9\% & 36.8\% & $+$21.1pp \\
\midrule
Overall    & 56.1\% & 36.9\% & $+$19.2pp \\
\bottomrule
\end{tabular}

\label{tab:gpqa_detail}
\end{minipage}
\hfill
\begin{minipage}{0.48\linewidth}
\centering
\small
\setlength{\tabcolsep}{4pt}
\caption{\textbf{Benchmark-dependent reversal for o3-mini vs.\ GPT-4o-mini.}
The reasoning-specialized model (o3-mini) outperforms the standard model on GPQA
Diamond ($+$19.2pp) but underperforms on IsoSci-150 ($-$24.7pp) and MMLU-STEM
($-$19.2pp). 
}
\vspace{4pt}
\begin{tabular}{lccc}
\toprule
\textbf{Benchmark} & \textbf{o3-mini} & \textbf{GPT-4o-mini} & $\Delta$ \\
\midrule
GPQA Diamond & 56.1 & 36.9 & $+$19.2 \\
IsoSci-150   & 36.8 & 61.5 & $-$24.7 \\
MMLU-STEM    & 60.0 & 79.2 & $-$19.2 \\
SciBench     & 41.7 & 38.5 & $+$3.2  \\
\bottomrule
\end{tabular}

\label{tab:benchmark_gpt}
\end{minipage}

\end{table}
 
% \begin{table}[h]
% \centering
% \caption{o3-mini vs.\ GPT-4o-mini accuracy breakdown on GPQA Diamond by domain.
% o3-mini substantially outperforms on physics and chemistry, confirming that
% reasoning helps on deep conceptual questions.}
% \label{tab:gpqa_detail}
% \small
% \begin{tabular}{lccc}
% \toprule
% \textbf{Domain} & \textbf{o3-mini} & \textbf{GPT-4o-mini} & $\Delta$ \\
% \midrule
% Physics    & 65.1\% & 44.2\% & $+$20.9pp \\
% Chemistry  & 47.3\% & 30.1\% & $+$17.2pp \\
% Biology    & 57.9\% & 36.8\% & $+$21.1pp \\
% \midrule
% Overall    & 56.1\% & 36.9\% & $+$19.2pp \\
% \bottomrule
% \end{tabular}
% \end{table}
 
\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{outputs/figure_1_domain_asymmetry.pdf}
\caption{\textbf{Domain-stratified accuracy deltas} (reasoning $-$ standard, pp) across
all three model pairs and four scientific domains, averaged over all benchmarks.
Left panel: per-pair deltas grouped by domain. Right panel: Spearman correlation between
average $\Delta_{\text{acc}}$ and domain computation intensity ($\rho=0.60$, $p=0.40$).
Error bars show 95\% bootstrap CIs. The toggle pairs (Qwen3-32B, Gemini 2.0 Flash)
show near-zero or small positive deltas; the traditional pair (o3-mini / GPT-4o-mini)
shows consistently negative deltas, reflecting that o3-mini trades broad knowledge recall
for deep reasoning capability.}
\label{fig:domain_asymmetry}
\end{figure}
 

 
This benchmark-dependent reversal has a direct implication: conclusions about
reasoning model utility on science depend entirely on which benchmark is used.
GPQA Diamond, with its emphasis on conceptual depth and multi-step derivation, favors
reasoning-specialized models. IsoSci-150, with its structured formula-substitution
problems, reveals that the same model is less capable of efficient knowledge retrieval.
Neither benchmark alone provides a complete picture; together they diagnose
\emph{where} and \emph{how} a model's science capability breaks down.
